Usable XAI: 10 Strategies Towards Exploiting Explainability in the LLM Era

Explainable AI (XAI) refers to techniques that provide human-understandable insights into the workings of AI models. Recently, the focus of XAI is being extended toward explaining Large Language Models (LLMs). This extension calls for a significant transformation in the XAI methodologies for two reasons. First, many existing XAI methods cannot be directly applied to LLMs due to their complexity and advanced capabilities. Second, as LLMs are increasingly deployed in diverse applications, the role of XAI shifts from merely opening the ``black box'' to actively enhancing the productivity and applicability of LLMs in real-world settings. Meanwhile, the conversation and generation abilities of LLMs can reciprocally enhance XAI. Therefore, in this paper, we introduce Usable XAI in the context of LLMs by analyzing (1) how XAI can explain and improve LLM-based AI systems and (2) how XAI techniques can be improved by using LLMs. We introduce 10 strategies, introducing the key techniques for each and discussing their associated challenges. We also provide case studies to demonstrate how to obtain and leverage explanations. The code used in this paper can be found at: https://github.com/JacksonWuxs/UsableXAI_LLM.

==> Figures/obs.tex <==
The expansion in the size of pre-trained language models has been considerable, with models encompassing billions of parameters. Such extensive growth has consistently showcased their capability to implicitly incorporate a wealth of human and factual knowledge~\citep{petroni2019language,li2022pre} within these parameters. Nonetheless, the lack of internal understandings towards LLM mechanisms results in limited efficacy in downstream tasks. In this section, we focus on three different levels of LLM internal interpretability, aiming to improve LLM performance with either \textit{fine-tuned} or\textit{ new-learnable} parameters. 


\subsection{Literature Review} 

Throughout this section, we denote the basic LLM as $f_{\theta}$, where $f$ can be generally represented by a function $f: \mathcal{X} \rightarrow \mathcal{Y}$, mapping from the input \textit{token} space to the \textit{output} prediction space. The research goal here is to update or modify the model parameters $\theta$ to achieve a better performance with $\theta^{*}$ for downstream tasks. To effectively and efficiently improve LLMs for particular predictions, internal interpretability on LLM mechanism can play an important role. Instead of fine-tuning $\theta$ from the whole, it is more preferable to identify the internal contributive components of LLMs first, and then modify or edit LLMs accordingly. In this section, we discuss the mechanical components of LLMs from three aspects, covering \textit{neurons}, \textit{layers} and \textit{modules}. The overall enhancement strategy for $f_\theta$ is to conduct localization or design before the tuning. 


\subsubsection{Neuron-wise Localization Methods} 

\textit{Neurons} are the most common focus of the localization analysis for LLM predictions. To localize the individual neuron which is responsible for model behaviors, \cite{mu2020compositional}, as one of the pioneers, identify the compositional logical concepts that closely approximate neuron behavior. Such neuron localization can not only identify abstractions and polysemanticity of the specific unit, but also disambiguate higher versus lower quality neurons in the model with respect to downstream performance. Following this direction, \cite{bolukbasi2021interpretability} further validate the encoding patterns of concepts for individual neurons within the BERT model, demonstrating how the geometry of BERT's activation space can influence the model performance. One step further, \cite{dai2022knowledge} investigates the contributive neurons, named as the \textit{knowledge neurons}, in pre-trained Transformers on relational fact storage, where the goal is to study the attributions between the neuron activations and the knowledge expression. The key insight from this work is that suppressing or amplifying the activation of knowledge neurons can accordingly alter the strength of knowledge expression, which is of great significance for downstream model improvement on generalization and robustness. As a more granular study, \cite{wang2022finding} focuses on the prompt-tuned pre-trained Transformers for specific tasks, and finds out that the ``\textit{skill}'' neurons extracted in pre-training stage do encode the useful patterns. When applying ``\textit{skill}'' neurons to network pruning~\citep{dalvi2020analyzing}, it is shown that the pre-trained LLM can be condensed up to 66.6\% of its initial parameters by exclusively maintaining the activity of the most proficient neurons, resulting in an approximate $1.4\mathrm{x}$ increase in inference speed. Also, for transferable soft prompt construction~\citep{su2022transferability}, the localized ``\textit{skill}'' neurons can bring about better performance regarding to the metric in \textit{overlapping rate} of activated neurons. Beyond the individual neurons, there are also some works~\citep{de2022sparse,casper2022graphical} exploring the groups of neurons for functional behaviors. Overall, neuron-wise localization aims to validate the neuron quality with activation patterns, so as to better improve the model performance by editing the components suggested by localization results. 


\subsubsection{Layer-wise Localization Methods} 

Different types of individual \textit{layers}, coupled with corresponding \textit{weight matrices}, serve as another important source for model localization and enhancement. In \cite{rogers2021primer}, a comprehensive study is conducted, showing the fact that BERT model is capable of storing syntactic, semantic and world knowledge within the its self-attention layers. In particular, the lower attention-layers contain the most information about linear word order~\citep{lin2019open}, and the syntactic information is most prominent in the middle attention-layers of BERT~\citep{hewitt2019structural}. As for the semantic and factual world knowledge, LLMs typically store them in the higher attention-layers, where an extra attentional hyper-network can be appended right before the decision stage for knowledge enhancement~\citep{de2021editing}. Besides, through the \textit{in-context} learning~\citep{wang2023label} and the \textit{dictionary} learning~\citep{cunningham2023sparse,bricken2023towards}, attentional layers within language models can be further modified and tuned to improve the LLM performance. Beyond attentional layers, regular MLP layers also show the evidences of their role in factual association and knowledge expression. In \cite{geva2021transformer}, the empirical studies show that feed-forward MLP layers emulate \textit{key-value memories}~\citep{sukhbaatar2019augmenting}, where keys are correlated with human-interpretable input patterns and values induce distributions over the output vocabulary that correlate with the next-token prediction. Such observation demonstrates the fact that 



\subsubsection{Module-wise Architecture Designs} 



\subsection{Challenges} 
Multi-modal knowledge, Continuous learning, Optimizing the efficiency


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> obsolete.tex <==
Explanations provide a lens through which we can assess whether a model's predictions are based on reasonable rationale. 
Let $x$ denote the input, $\hat{y}=f(x)$ be the target model's output, and $\mathbf{a}\in \mathbb{R}^{N\times M}$ be the attribution score matrix.
The goal is to construct a diagnostic classifier $g_{\mathrm{diag}}(\mathbf{a}, x, \hat{y}) \in \{-1, +1\}$ where $+1$ indicates that the prediction is trustworthy, while $-1$ means the opposite.
A general pipeline that leverages attribution scores to analyze LLM behaviors is shown in Figure~\ref{fig:attribution_pipeline}. 
In this approach, $\mathbf{a}$ is incorporated as \textbf{additional features}.
Typically, $g_{\mathrm{diag}}$ can be implemented as a lightweight model or another LLM. 
% First, given the target LLM and an input prompt, we compute attribution scores of input-output token pairs.
% Second, we extract a feature vector from the attribution map, tailored to the requirements of the diagnostic task at hand.
% Third, a light-weight predictor is trained to diagnose whether the model behaves appropriately based on the feature vector.
In the following, we provide case studies to illustrate how attribution scores could be utilized to assess LLM response quality.
% ~\citep{adlakha2023evaluating}. 


\subsubsection{LLM Response Quality Evaluation with Explanations}
This case study explores the use of attribution-based explanations as evidence to assess the quality of LLM-generated responses. 
Here, ``quality'' is specifically measured by the responses' accuracy. 
We hypothesize that responses generated from correct rationales are likely to be more accurate. 
%Our method involves comparing the model's explanations with underlying rationales as a means to evaluate response accuracy. 
Verifying the quality of responses is crucial for applications such as medical chat systems.


\paragraph{Experimental Design.} 
This case study uses the MultiRC dataset~\citep{khashabi2018looking}, which requires the model to answer questions grounded on multiple sentences from a given paragraph. 
%The answers may not directly correspond to specific sentence spans, reflecting a more realistic scenario of modern LLMs. 
Each MultiRC instance is associated with a human-annotated rationale indicating which sentences are relevant for answering the question. Our study specifically employs its test subset with 950 samples in total. We consider 80\% of which as the training set and report the results on the remaining samples.  
We focus on the Vicuna-7B model~\citep{chiang2023vicuna}, and apply the Normalized Importance Density Score method~\citep{wu2023language} to estimate the importance of each word in the provided paragraph. 
%Specifically, given $N$-word paragraph $X$ and the $M$-word response $\hat{Y}$, the attribution from each input word $x_n$ to each output word $\hat{y}_m$ is defined as $a_{n,m} = \frac{\partial f(y_m|Z_m)}{\partial\,\mathbf{E}_i[x_n]}\cdot \mathbf{E}_i[x_n]^\top$, where $Z_m$ indicates the formatted input prompt concatenated with the first $m-1$ response word, $f$ is the language model, and $\mathbf{E}_i[x_n]$ indicates the input static embedding of $x_n$. This pairwise attribution score is then normalized as $\widetilde{a}_{n,m}=\lceil L\times a_{n,m} / \text{max}_{n'}(a_{n',m})\rceil$. Any normalized attribution $\widetilde{a}_{n,m}$ is equal or less than $b$ will is forced to 0. The overall attribution score on word $x_n$ is defined as its attribution density, i.e., $a_n=||[a_{n,1},...,a_{n,M}||_1 / ||[a_{n,1},...,a_{n,M}]||_p$. In our experiments, we let $L=10$, $b=2$, $p=5$, and consider Vicuna-7B-v1.1 as our language model $f$. By averaging these word attribution scores, we reach the importance of each sentence. 
The top-K sentences with the highest importance scores are selected as the explanation for each instance, which is then fed to a classifier to predict whether Vicuna's outputs are correct. The classifier is initialized with DistillBERT-base~\citep{sanh2019distilbert}, and fine-tuned on the training set. We also consider the original full paragraph or the human-annotated rationales as the explanation part to train the classifiers as our baselines. 
Following previous studies~\citep{khashabi2018looking,deyoung2019eraser}, we evaluate the accuracy of each response by exactly matching all correct answers within the responses. 
Table~\ref{tbl_quality} reports the macro precision, recall, F1, and AUC scores on the test set.

\paragraph{Results.} 
\begin{wraptable}{r}{0.48\textwidth}
\small
\centering
\vspace{-0.6cm}
\caption{Utilizing attribution for response quality evaluation}
\label{tbl_quality}
\vspace{-0.4cm}
\begin{tabular}{lcccc}
\toprule
Setting             & Precision & Recall & F1    & AUC   \\ 
\midrule
Random & 49.40    & 51.79  & 49.61 & 49.03 \\
\midrule
Human Rationale            &    68.73       &   66.88  &   67.57   &   73.11    \\
Full Paragraph          &  58.02    & 58.47 & 56.89 & 63.44 \\
Attribution (ours)          &    63.25     & 67.69  & 64.12   & 71.53 \\
\bottomrule
\end{tabular}
\vspace{-0.4cm}
\end{wraptable}
Table~\ref{tbl_quality} shows that isolating the rationales from the full context could best help the classifier identify the response quality. 
%We could also observe that providing machine explanations to the classifier could reach a performance closely matching the human-annotated rationales, indicating the machine-generated explanations maintain a strong quality with the human rationales. 
%Table~\ref{tbl_quality} presents the quality of explanations, categorized based on the accuracy of the corresponding responses. 
%It is evident that explanations align more closely with human-annotated rationales when associated with correct responses. 
In addition, the precision and recall metrics for explanations derived from correct answers surpass those associated with incorrect responses. This finding serves as empirical evidence underscoring the effectiveness of attribution-based explanations in estimating the accuracy of responses generated by LLMs.


\subsubsection{Hallucination Detection with Attribution Explanations}
This case study explores a different aspect of LLM generation quality, focusing on the presence of \textit{hallucinations} in LLM-generated responses. 
Hallucinations are defined as responses that contain information conflicting with or unverifiable by factual knowledge~\citep{li2023halueval,ji2023survey}. 
%For instance, if a model is asked about a fictitious entity like ``King Renoit'' and responds with a narrative about ``The Three Musketeers'', claiming it pertains to the nonexistent king, it illustrates a hallucination. 
%This tendency, particularly pronounced in instruction-tuned models, stems from their earnest endeavor to fulfill user requests. 
The issue often arises when direct commands (``tell me a story'') significantly influence the generation process, while the instruction's subject (``about King Renoit'') is neglected. 
We show that attribution-based explanation over different types of prompting words can serve as an indicators to detect LLM hallucinations. 
% Based on this insight, we develop a hallucination detector according to the distribution of attribution scores over different types of prompting words. 

\paragraph{Experimental Design.}
We use the Hallucination Evaluation Benchmark~\citep{li2024dawn} in this case study. Each instance includes an input prompt, a ChatGPT~\citep{ouyang2022training} response, and the correlated knowledge. %Each piece of knowledge has been annotated about whether it is true. 
Each instance having at least one invalid knowledge is considered a hallucination response. This study focuses on 632 less confused samples, each of which has almost all knowledge correct or wrong. We randomly select 80\% of the selected samples for training and the rest for testing. 
%Given a prompt and its ChatGPT response, we build a classifier to detect if the response is hallucinated.
We apply Vicuna-7B~\citep{chiang2023vicuna} and Mistral-7B~\citep{jiang2024mixtral} to compute the Normalized Importance Density Scores~\citep{wu2023language} over each prompt-response instance pair. 
We also identify part-of-speech (POS) tags of each prompting word with NLTK~\citep{loper2002nltk}. 
Finally, we construct a 82-dimensional vector for each instance, where each dimension indicates the average attribution scores over a certain type of POS tagging. 
We train a Support Vector Machine based on the constructed vectors and report its precision, recall, and F1 scores on the hallucination samples, as well as accuracy over all samples in Table~\ref{tbl_hallucination}. 
We also leverage a fine-tuned~\citep{chern2023factool} and a prompting-based~\citep{li2024dawn} baselines. 


\paragraph{Results.}
\begin{wraptable}{r}{0.6\textwidth}
\small
\centering\vspace{-0.15cm}
\caption{Utilizing attribution for hallucination detection on ChatGPT responses.}
\vspace{-0.2cm}
\label{tbl_hallucination}
\begin{tabular}{@{}c|c|cccccc@{}}
\toprule
Method & LLM             & Precision & Recall & F1  & Accuracy   \\ 
\midrule
Random &     -      &      88.41     &    50.34    &    64.11  &   50.59 \\
FacTool       & GPT-4           &      95.30   &  72.93     &   82.62 & 73.04 \\
Vectara      & DeBERTa-base      &  90.29     & 60.54 & 72.40 & 59.45 \\
\midrule
AttrScore    & Vicuna-7B & 90.15       &  74.21 & 81.36 & 70.20 \\
           (ours)          & Mistral-7B &  88.74   & 75.04 &  81.26  & 69.57 \\
\bottomrule
\end{tabular}
\vspace{-0.6cm}
\end{wraptable}
% \begin{table*}[t]
% \small
% \centering
% %\vspace{-0.4cm}
% \caption{Utilizing attribution for hallucination detection on ChatGPT responses.}
% \vspace{-0.4cm}
% \label{tbl_hallucination}
% \begin{tabular}{l|c|cccccc}
% \toprule
% Method & Language Model             & Precision & Recall & F1  & Accuracy   \\ 
% \midrule
% Random &     -      &      88.41     &    50.34    &    64.11  &   50.59 \\
% FacTool       & GPT-4           &      95.30   &  72.93     &   82.62 & 73.04 \\
% Vectara      & DeBERTa-base      &  90.29     & 60.54 & 72.40 & 59.45 \\
% \midrule
% \multirow{2}{*}{AttrScore (ours)}    & Vicuna-7B & 90.15       &  74.21 & 81.36 & 70.20 \\
%                     & Mistral-7B &  88.74   & 75.04 &  81.26  & 69.57 \\
% \bottomrule
% \end{tabular}
% \vspace{-0.4cm}
% \end{table*}
In the table, we first observe that all methods have demonstrated a greater performance than the Random strategy. 
In addition, we observe that the proposed methods achieve a competitive performance with FacTool using GPT-4, establishing a new benchmark in this domain. It is worth noting that, instead of using GPT-4, the attribution score for our method is calculated using a smaller 7-billion-parameter language model. This demonstrates the practicality and efficiency of our approach in \textit{weak-to-strong generalization} as we could diagnose large language models with smaller models. 
%Future work could consider extracting more effective features and using more powerful classifiers.

\subsection{Explanation-guided Data Augmentation for Mitigating Shortcuts}
Machine learning models are prone to make predictions with spurious correlations~\citep{geirhos2020shortcut}, which are misaligned with human reasoning processes. This dependency on shortcuts notably diminishes a model's ability to generalize to out-of-distribution samples and weakens its resilience against adversarial attacks~\citep{xu2020adversarial}. Essentially, if a model's predictions are predominantly based on shortcut features, it indicates that the underlying mechanisms of the model are not interpretable from a human perspective.
Therefore, post-hoc explanation techniques play a crucial role in detecting undesirable correlations between input and predictions~\citep{liu2018adversarial,liu2021adversarial}. For example, \citet{du2021towards} adopt Integrated Gradient (IG) to attribute a model's predictions to its input features, showing that the model tends to treat functional words, numbers, and negation words as shortcuts and rely on them for prediction in natural language understanding tasks. 


Data augmentation can be applied to train models that are less sensitive to shortcut features. Explanatory information such as counterfactuals~\citep{wang2021robustness} has been incorporated to improve model robustness. 
This method can also be extended to enhance the out-of-distribution performance of smaller models using LLMs as generators~\citep{sachdeva2023catfood}. For example, LLMs are able to synthesize rare examples, which helps smaller models generalize better on unseen data~\citep{xu2023contrastive}.  
Besides, LLMs are promising in improving model safety by generating more natural adversarial examples compared to conventional approaches~\citep{wang2023generating}. First, the most vulnerable words are identified using attribution-based methods. Then, LLMs generate candidates similar to identified words. These candidates are filtered by an external classifier. Subsequently, these adversarial examples are used to train downstream models to boost their security.
Similarly, LLMs are also helpful in mitigating biases such as fairness issues in models~\citep{he2023targeted}. This work claims that it automatically identifies underrepresented subgroups, and chooses an optimal augmentation strategy that avoids hurting other groups. New group examples are generated using LLMs with human-provided labels. The experiments observe improvements in both underrepresented groups and overall model performance. 

\subsection{Explanation-enhanced Data Enrichment}
LLMs have been leveraged to directly generate natural language explanations as augmented data. This strategy relies on the understanding capabilities of LLMs to assist smaller models in their learning tasks.~\citet{li2022explanations} introduce LLM explanations to facilitate the training of smaller models, which improves their reasoning capabilities and acquires explanation generation abilities. With the best-case scenario in a reasoning task, a 9.5\% improvement on accuracy compared to 60x larger GPT-3 has been observed~\citep{li2022explanations}. It is worth noting that LLMs including ChatGPT and GPT-4 are competitive in generating coherent and logical explanations, except for limited languages~\citep{whitehouse2023llm}. 
LLM explanations have also been utilized to mitigate spurious correlations in aspect-based sentiment analysis tasks~\citep{wang2023reducing}. This study proposes using LLMs to generate explanations for sentiment labels of aspects in sentences~\citep{wang2023reducing}. These explanations help models to reason with contextual semantics rather than spurious correlations, making the model more robust and improving both in-domain performance and generalization ability~\citep{wang2023reducing}.
Another line of work involves integrating LLM rationales as additional supervision to guide the training of smaller models. Experiments have shown that this approach not only requires fewer training data but also outperforms traditional fine-tuning and distillation methods~\citep{hsieh-etal-2023-distilling}.

In addition to the aforementioned augmentation techniques, we envision several potential applications in enhancing model performance. For example, one promising application lies in guiding the parameter learning of small models by using automatically generated explanations. Previous research has investigated this avenue by directing the attention of models towards human-crafted explanations~\citep{stacey2022supervising}. Thus, LLMs can replace human as generators presenting a more economic and versatile alternation. Another potential application is to enhance model performance on complex tasks using natural language explanations from LLMs. For instance, code translation generation tasks incorporate explanations as an intermediate step, improving model performance by 12\% on average~\citep{tang2023explain}. The result shows that explanations are particularly useful in zero-shot settings. Apart from assisting in smaller models, LLMs have demonstrated their ability to improve their own reasoning abilities by generating reliable rationales~\citep{huang2022large}.
